Maximum Regularized Likelihood Estimators: A General Prediction Theory and Applications

Maximum regularized likelihood estimators (MRLEs) are arguably the most established class of estimators in high-dimensional statistics. In this paper, we derive guarantees for MRLEs in Kullback-Leibler divergence, a general measure of prediction accuracy. We assume only that the densities have a convex parametrization and that the regularization is definite and positive homogenous. The results thus apply to a very large variety of models and estimators, such as tensor regression and graphical models with convex and non-convex regularized methods. A main conclusion is that MRLEs are broadly consistent in prediction - regardless of whether restricted eigenvalues or similar conditions hold.

==> Sections/Framework.tex <==

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 

\section{Framework and Notation}
In this paper, we introduce a general framework for graphical models. This framework encompasses the standard types of graphical models as well as new types of graphical models. In particular, the framework allows for the inclusion of Poisson and exponential data and for transformations and combinations of such data. Moreover, we show that maximum likelihood provides consistent estimation and inference for the model parameters in the framework. 

\subsection{Notation} We equip matrices in $\R^{p \times p} $ with the trace inner product 
\begin{align*}
	\inprodtr{\cdot}{\cdot}:\R^{p \times p} \times \R^{p \times p} \to&\ \R\\
	(A, B)\mapsto&\ \inprodtr{ A}{ B}:=\sum_{i,j=1}^p A_{ij} B_{ij}
\end{align*}
and the associated norm
\begin{align*}
	\normtr{\cdot}:\R^{p \times p}  \to&\ [0,\infty)\\
	A \mapsto&\ \sqrt{\inprodtr{ A}{A}}= \sqrt{\sum_{i,j=1}^p A_{ij}^2 }\ .
\end{align*}

Consider random vectors $X=(X_1, \cdots X_p)^T \in \R^p$. We denote random vectors and their realizations by the upper case letter X and arguments of functions by the lower case, boldface letter \textbf{x}. For given $i, j \in \{1,2,\cdots, p\}$ and $i \neq j$, independence of two elements $X_i$ and $X_j$ is denoted by $X_i \perp X_j$; conditional independence of $X_i$ adn $X_j$ given all other elements is denoted by $X_i \bigCI X_j \mid X_{-\{i,j\}}$.

For given symmetric $\matrix \in \R^{p \times p}$ and index $j\in\{1,\dots,p\},$ we set $\nbj:=\{i\in\{1,\dots,p\}:i \neq j, \matrix_{ij} \neq 0\}$ as the neighborhood of node $j$.

\subsection{Exponential Trace Models}\label{sec:model} In this section, we introduce a probabilistic framework to model vector-valued observations with dependent coordinates. Specifically, we consider an arbitrary (non-empty) $\Domain$ and random vectors $X\in\Domain$ that have densities of the form
\begin{equation}\label{eqn: exponential trace model}
f_\matrix(\textbf{x}):=e^{-\inprodtr{\matrix}{T(\textbf{x})}+\hterm\left(\datav\right)-\normtotal(\matrix)}
\end{equation}
with respect to some $\sigma$-finite measure \measure\ on \Domain. We call these models {\it exponential trace models}.

The densities are indexed by $\matrix \in \Matrix$, where $\Matrix$ is a non-empty, open set of symmetric elements in~$\R^{p \times p}.$ The data enters the model via a matrix-valued mapping
\begin{align*}
	T:\Domain\to&\ \R^{p \times p}\\
	\datav\mapsto&\ T(\datav)\,,
\end{align*}
and via a function \hterm
\begin{align*}
	\hterm:\Domain\to&\ \R\\
	\datav\mapsto&\ \hterm(\mathbf{\datav}).
\end{align*}
The quantity~$\normtotal(\matrix)$ is finally the normalization defined as
\begin{equation*}
	\normtotal(\matrix):=\log\int_\Domain e^{-\inprodtr{\matrix}{T(\datav)}+\hterm(\datav)}\,d\measure\,.
\end{equation*}
To obtain well-defined families of densities, we assume that $\Matrix$ is an open, convex subset of matrices in $\Matrix^*$, where for given $\Domain, T, \hterm$, 
\begin{equation*}
	\Matrix^* := \text{interior}\{\matrix \in \R^{p \times p}: \normtotal(\matrix) < \infty\}.
\end{equation*}
The set $\Matrix$ is the parameter space deemed suitable for a given application, while the set $\Matrix^*$ is the largest possible parameter space compatible with our framework. 

\subsection{Estimation Procedure}\label{sec:estimator} For this, we assume that the model (1) holds for an  $\matrixtrue\in\Matrix$. Our goal is then to estimate $\matrixtrue$ given $n$ i.i.d. copies of $\datav$ denoted by $\datasseq$. We first summarize these data in the  generalized Gram matrix 
\begin{equation*}
	\overline{T}\equiv \overline{T}(\datasseq):=\sino T(X^i)\,. 
\end{equation*}
The negative joint log-likelihood according to the model (1) is then
\begin{equation*}
	-\ell_\matrix(\datasseq):= n\inprodtr{\matrix}{\overline{T}}-\si\hterm(\datasi)+n\normtotal(\matrix)\, .
\end{equation*}
For further reference, we state the essence of this in the following lemma.
\begin{lemma}[Log-likelihood]
	Given any $\matrix\in\Matrix^*$,  the negative joint log-likelihood~$-\ell_\matrix$ for the observed data $\datasseq$ can be expressed as 
	\begin{equation*}
		-\ell_\matrix(\datasseq)= n\inprodtr{\matrix}{\overline{T}}+n\normtotal(\matrix)+c\, ,
	\end{equation*}
	where $c\in\R$ does not depend on $\matrix.$
\end{lemma}

Motivated by Lemma 1.1, we introduce an estimator of \matrixtrue\ by
\begin{equation*}
	\widehat{\matrix}:=\argmin_{M\in\Matrix}\left\{-\ell_\matrix(\datasseq)\right\}=\argmin_{M\in\Matrix}\left\{\inprodtr{\matrix}{\overline{T}}+\normtotal(\matrix)\right\}.
\end{equation*}
The objective function underlying this estimator has two important properties. First, it is convex:
\begin{lemma}[Convexity]\label{convexity}
	For any $\datasseq\in\Domain,$ the function
	\begin{align*}
		\Matrix^*\to&\ \R\\
		M\mapsto&\ \inprodtr{\matrix}{\overline{T}}+\normtotal(\matrix)
	\end{align*}  
	is convex.
\end{lemma}
\noindent Second, its derivatives can be computed explicitly.
\begin{lemma}[Derivatives]\label{derivative}
	For any $\datasseq\in\Domain,$ the function
	\begin{align*}
		\Matrix^*\to&\ \R\\
		\matrix\mapsto&\ \inprodtr{\matrix}{\overline{T}}+\normtotal(\matrix)
	\end{align*}  
	is twice differentiable with partial derivatives
	\begin{equation*}
		\frac{\partial}{\partial \matrix_{ij}}\left(\inprodtr{\matrix}{\overline{T}}+\normtotal(\matrix)\right)= \overline{T}_{ij}-\mathds{E}_\matrix\overline{T}_{ij}
	\end{equation*}
	and
	\begin{align*}
		&\frac{\partial}{\partial \matrix_{ij}}\frac{\partial}{\partial \matrix_{i'j'}}\left(\inprodtr{\matrix}{\overline{T}}+\normtotal(\matrix)\right)\\
		&~~~~~~~~~~~~~~~~~~~=n\E_\matrix\left[\big(\overline{T}_{ij}-\mathds{E}_\matrix\overline{T}_{ij}\big)\big(\overline{T}_{i'j'}-\mathds{E}_\matrix\overline{T}_{i'j'}\big)\right]
	\end{align*}
	for $i,j,i',j'\in\otp\,.$
\end{lemma}
\noindent \noindent Convexity and the explicit derivatives are desirable for both optimization and theory. From a optimization perspective, the two properties are important, because they render the objective function amenable to gradient-type minimization. From a theoretical perspective, the two properties are imporant, because they  imply that
\begin{equation*}
	\matrixtrue=\argmin_{\matrix\in\Matrix}\left\{\E_{\matrixtrue}\left(\inprodtr{\matrix}{\overline{T}}+\normtotal(\matrix)\right)\right\}\,,
\end{equation*}
showing that $\widehat{\matrix}$\ is indeed a standard M-estimator. 

\subsection{Asymptotic Normality}\label{sec:normality} We now show that the M-estimator is asymptotically normal with covariance equal to the Fisher information. This  allows for the construction of efficient asymptotic tests and confidence sets.

The asymptotic normality of the estimator is established in the following result.
\begin{theorem}\label{normality}
	The estimator $\widehat{\matrix}$ is asymptotically normal with covariance equal to the Fisher information. 
\end{theorem}

\noindent This results implies in particular that the estimator is asymptotically efficient~\cite[Chapter~4.5]{Shao03}.

\begin{remark} 
	The Fisher information $I_\matrix$ is given by 
	\begin{equation*}
		(I_\matrix)_{ijkl} = n\mathds{E}\big[\big(\overline{T}_{ij}-\mathds{E}_\matrix\overline{T}_{ij}\big)\big(\overline{T}_{kl}-\mathds{E}_\matrix\overline{T}_{kl}\big)\big]
	\end{equation*}
	for $i,j,k,l \in \{1,\cdots, p\}$. This explicit expression can be used to show three important properties: (i) It can be used to show that $I_\matrix$ is invertible. (ii) It can be used to show that the density with respect to the Lebesgue measure of the normal distribution with mean zero and covariance equal to the Fisher information has a concise form. Indeed, we find that the density as a function of $A \in \R^{p \times p}$ is proportional to
	\begin{equation*}
		e^{-\mathds{E}_\matrix\inprodtr{A}{T-\mathds{E}T}^2/2}.
	\end{equation*}
	this formulation highlights once again the prominent role of the trace in our framework. (iii) Finally, it can be used to show that for decomposable models, the non-zero pattern in $\matrix$ not only determines the dependencies among the coordinates of X but also the asymptotic dependencies among the coordinates of \matrix  . Most illustrative for this is the case where $\matrix$ is diagonal, that is, the coordinates of $\matrix$ are independent. Then, the above expression implies that $I_\matrix$ is diagonal, so that also the coordinates of $\matrix$  are asymptotically independent.
\end{remark}	
